Spectral stability of V2 centres in sub-micron 4H-SiC membranes

Colour centres in silicon carbide emerge as a promising semiconductor quantum technology platform with excellent spin-optical coherences.However, recent efforts towards maximising the photonic efficiency via integration into nanophotonic structures proved to be challenging due to reduced spectral stabilities. Here, we provide a large-scale systematic investigation on silicon vacancy centres in thin silicon carbide membranes with thicknesses down to $0.25\,\rm\mu m$. Our membrane fabrication process involves a combination of chemical mechanical polishing, reactive ion etching, and subsequent annealing. This leads to highly reproducible membranes with roughness values of $3-4\,\rm\r{A}$, as well as negligible surface fluorescence. We find that silicon vacancy centres show close-to lifetime limited optical linewidths with almost no signs of spectral wandering down to membrane thicknesses of $0.7 \,\rm\mu m$. For silicon vacancy centres in thinner membranes down to $0.25\,\rm\mu m$, we observe spectral wandering, however, optical linewidths remain below $200\,\rm MHz$, which is compatible with spin-selective excitation schemes. Our work clearly shows that silicon vacancy centres can be integrated into sub-micron silicon carbide membranes, which opens the avenue towards obtaining the necessary improvements in photon extraction efficiency based on nanophotonic structuring.

==> texts/old_intro.tex <==
Optically-active spin defects in solids promise a variety of applications in the field of quantum technologies \cite{Awschalom2018}.
While the negatively charged nitrogen-vacancy centre (NV$^{-}$) in the diamond lattice has been used as the prime candidate in this field, enabling breakthrough experiments for quantum sensing \cite{Mamin2013, Aslam2017}, scalable quantum information processing \cite{Robledo2011, Waldherr2014, Bradley2019}, and quantum communication \cite{Togan2010, Bernien2013, Pompili2021}, silicon carbide (SiC) has currently emerged as an alternative host for quantum emitters \cite{Son2020, Castelletto2020}.
Compared to diamond, it offers complementary metal-oxide-semiconductor (CMOS) compatibility \cite{Liu2015} and commercial availability of the material on wafer-scale \cite{Blevins2020}, both desirable for the scalability of the system.
% Maybe one sentence that includes polytypes

Recent studies have identified divacancy centres (V$_{\mathrm{C}}$V$_{\mathrm{Si}}$) \cite{Christle2017} and silicon-vacancy centres V$_\mathrm{Si}^{-}$ in 4H-SiC \cite{Nagy2019} as suitable emitters for high-fidelity spin-photon interfaces.
%For V$_{\mathrm{Si}}$ in epitaxial grown 4H-SiC films, near Fourier-limited linewidths \cite{Nagy2019, Morioka2020, Babin2022}, a small inhomogeneous distribution of the zero-phonon-lines (ZPLs) of different emitters \cite{Nagy2021}, photon indistinguishability \cite{Morioka2020}, and spin coherence exceeding \SI{1}{\milli\second} \cite{Kraus2017, Babin2022}, have already been demonstrated.
However, like in diamond the high refractive index of SiC leads to total internal reflection at the crystal interface, reducing the collection efficiency of photons emitted from optically-active spin defects \cite{Siyushev2010}. % Additional reference for SiC?!
Additionally, the presence of a dark intersystem crossing further degrades the rate of emitted photons \cite{Fuchs2015,Singh2022}. 

Photonic structuring of the host crystal in the vicinity of emitters provides a possible solution to those challenges \cite{Janitz2020, Lukin2020Integrated, Castelletto2021}.
For different emitters in SiC, an increase in the collection efficiency was demonstrated using nanopillars \cite{Radulaski2017} and solid immersion lenses \cite{Sardi2020}, while photonic resonators were implemented to Purcell enhance their emission in the ZPL \cite{Bracher2017, Lukin2020, Crook2020, Lukin2023}.
In this context, the use of thin films is of particular interest, since it offers the potential for integrated photonics \cite{Bogaerts2004, Ye2013, Siew2021} or hybrid photonic structures \cite{Weigel2016, He2019} and has been already successfully adapted from silicon photonics with the silicon-carbide-on-insulator platform \cite{Lukin2020, Wang2021}.
Furthermore, as shown for other host materials, (sub-)µm-thin films, which we will refer to as membranes in this manuscript, offer alternative approaches, such as planar optical antennas \cite{Lee2011, Fuchs2021} or external Fabry-Pérot cavities \cite{Riedel2017, Haeussler2019, Salz2020, Ruf2021} to improve the photon extraction.

The challenging preservation of the optical coherence of quantum emitters in nanofabricated structures, i.e. maintaining nearly-lifetime limited optical absorption linewidths throughout the fabrication, has been demonstrated recently for suspended structures in bulk material \cite{Babin2022} as well as in thin film SiC \cite{Lukin2023}.
However, the results from \cite{Babin2022} indicate a reduction of the emitter density after the fabrication and a study focusing on the effects of different fabrication steps is missing so far to the best of our knowledge, yet could give helpful insights towards scalable integration of optically coherent emitters in SiC nanostructures. 

In our work, we fabricate membranes from 4H-SiC with minimum thicknesses between \SIrange{0.14}{2.36}{\micro\meter} and study the emission of pre-fabrication created V$_\mathrm{Si}^{-}$ centres inside these membranes.
Moreover, we perform photoluminescence-excitation (PLE) measurements on V2-centres, i.e. silicon vacancy centres at the cubic lattice site \cite{Ivady2017}, to probe their optical absorption linewidths for different membrane thicknesses and fabrication steps. We find emitters with PLE-linewidths below \SI{200}{\mega\hertz} within membranes of \SIrange{0.25}{2.05}{\micro\meter} thickness and a clear trend of an increased spectral wandering of the PLE center frequencies for thinner structures, while we identify several emitters in \SI{\sim0.65}{\micro\meter}-thick membranes with only weak signs of wandering. Our results strongly motivate the use of the membrane integrated V$_\mathrm{Si}^{-}$ for the above mentioned photonic structures, while further studies seem necessary to fully understand the decrease in the density of optically-coherent emitters during fabrication and to find ways for improved preservation of the optical coherence.

